Towards Accelerated Greedy Sampling and Reconstruction of Bandlimited Graph Signals

We study the problem of sampling and reconstructing spectrally sparse graph signals where the objective is to select a subset of nodes of prespecified cardinality that ensures interpolation of the original signal with the lowest possible reconstruction error. This task is of critical importance in Graph signal processing (GSP) and while existing methods generally provide satisfactory performance, they typically entail a prohibitive computational cost when it comes to the study of large-scale problems. Thus, there is a need for accelerated and efficient methods tailored for high-dimensional and large-scale sampling and reconstruction tasks. To this end, we first consider a non-Bayesian scenario and propose an efficient iterative node sampling procedure that in the noiseless case enables exact recovery of the original signal from the set of selected nodes. In the case of noisy measurements, a bound on the reconstruction error of the proposed algorithm is established. Then, we consider the Bayesian scenario where we formulate the sampling task as the problem of maximizing a monotone weak submodular function, and propose a randomized-greedy algorithm to find a sub-optimal subset of informative nodes. We derive worst-case performance guarantees on the mean-square error achieved by the randomized-greedy algorithm for general non-stationary graph signals.

==> Secrec.tex <==
In the previous sections, we assumed that the support of the bandlimited graph signal $\x$ (that is, the set of 
nonzero frequency components) is known. However, in many practical settings, the support of the signal might 
be unknown and one needs to recover it prior to or concurrent with the sampling step. In this section, we 
address this task and provide a novel framework to efficiently identify the support. 

%The problem of the identifying the support of the graph signal is considered in \cite{marques2016sampling} where authors prove that if all eigenvalues of the graph shift operator (adjacency $\A $ or  the Laplacian $\mathbf{L}$ defined as $\mathbf{L} = \text{diag}(\mathbf{A}\mathbf{1}_{N}) - \mathbf{A}$, for example) are distinct and nonzero, and under certain conditions on sampling matrix  $\C$, the aggregation sampling method can recover the unknown support of a $k$-sparse graph signal from $m = 2k$ noiseless samples. Compared to  the case where the support $\K$ is known, the aggregation sampling method of \cite{marques2016sampling} requires twice as many samples as the bandwidth of the graph signal (i.e., $k$) for perfect recovery of $\K$ and hence exact interpolation of $\x$ from the sampled signal $\hat{\x}$. The conditions under which exactness of aggregation sampling is guaranteed might be strong in practical setting where the graph is arbitrary.

Existing selection and aggregation sampling methods capable of support identification (e.g. \cite{marques2016sampling}) require twice as many samples as the bandwidth of the graph signal (i.e., $k$) for perfect recovery of $\K$ and hence exact interpolation of $\x$ from the sampled signal $\hat{\x}$. Furthermore, the conditions needed to ensure exactness 
of aggregation sampling may be challenging to meet in practical setting where the graph is arbitrary. % See Fig.~\ref{fig:simple} for an illustrative example.

%For example, in undirected graphs, common choice of graph shift operator is combinatorial Laplacian $\mathbf{L}$. Consider all six possible unweighted and unlabeled undirected graphs with $N=4$ nodes shown in Fig.~\ref{fig:simple}. It should be noted that for any labeling, eigenvalues of $\mathbf{L}$ remain the same. Finding the eigenvalues of the Laplacian for the graphs in Fig.~\ref{fig:simple} reveals that only two out of the six graphs meet the condition of eigenvalues being distinct (the two leftmost graphs), a necessary condition required by \cite{marques2016sampling} for support identification. However, the matrix of eigenvectors for $\mathbf{L}$ can be found to be full rank and orthogonal in all cases.

%In fact even for the extremely simple unweighted graph illustrated in Fig. \ref{fig:simple}, the conditions stated in \cite{marques2016sampling} are not met. For the graph in Fig. \ref{fig:simple}, it holds that 
%\begin{equation}
%\A = \left[
%\begin{matrix}
%0 & 1&0&0 \\
%1 & 0&0&0 \\
%0 & 0&0&1 \\
%0 & 0&1&0 \\
%\end{matrix}
%\right], \quad
%\mathbf{L}
%\left[
%\begin{matrix}
%1 & -1&0&0 \\
%-1 & 1&0&0 \\
%0 & 0&1&-1 \\
%0 & 0&-1&1 \\
%\end{matrix}
%\right].
%\end{equation}
%If we find the eigenvalue decomposition $\A = \V \mathbf{\Lambda}\V^\top$, we notice that $\mathbf{\Lambda} = \mathrm{diag}(1,1,-1,-1)$. Also, finding the eigenvalue decomposition $\mathbf{L} = \V_L \mathbf{\Lambda}_L\V_L^\top$ reveals that $\mathbf{\Lambda}_L = \mathrm{diag}(2,2,0,0)$. Moreover both $\V$ and $\V_L$ are full rank, orthogonal matrices. Hence, it is easy to see that aggregation sampling will fail in this simple example as the conditions stated in \cite{marques2016sampling} are not met.
%\begin{figure}[t]
%	\begin{minipage}[b]{\linewidth}
%		\centering
%	%	\includegraphics[width=0.3\textwidth]{Figures/simple.png}
%		\includegraphics[width=1\textwidth]{Figures/4-node.eps}
%		%\centerline{(a)}\medskip
%	\end{minipage}
%	\caption{All six possible unweighted and unlabeled undirected graphs with $4$ nodes along with their corresponding eigenvalues underneath. The aggregation sampling \cite{marques2016sampling} fails to identify the unknown support of the graph signal supported on the four rightmost illustrated graphs due to the repetitive eigenvalues.}
%	\label{fig:simple}
%	%\vspace{-0.5cm}
%\end{figure}
Here we propose a support recovery approach for a broad range of graphs. Then we combine the support 
recovery and sampling schemes of the previous sections into an adaptive graph sampling with support 
identification framework.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\vspace{-0.3cm}
\subsection{Support recovery from historical signals}\label{sec:rec_hist}
Suppose that for a given graph and its Fourier basis $\mathbf{V}$, the observed $P$ signals measured at all 
of the $N$ vertices are collected in a matrix $\mathbf{Y} = [\mathbf{y}^{1}, \cdots, \mathbf{y}^{P}] \in 
\mathbb{R}^{N \times P}$. The goal is to perform support recovery of the underlying bandlimited signals collected 
in $\mathbf{X} = [\mathbf{x}^{1}, \cdots, \mathbf{x}^{P}] \in \mathbb{R}^{N \times P}$ which involves estimating 
sparse GFTs $\bar{\mathbf{X}} = [\bar{\x}^{1},\cdots,\bar{\x}^{P}] = \mathbf{V}^{-1} \mathbf{X}$. We assume that 
$\mathbf{V}$ has full rank and that GFTs $\bar{\mathbf{x}}^{i}$ share a common support. 
{\color{black}{Note that the latter assumption means that matrix 
$\bar{\mathbf{X}}$ is a  block-sparse matrix having entire rows as zeros or nonzeros.}} 
Recall that $\mathcal{K}$ is the support set of GFTs $\bar{\mathbf{x}}^{i}$ with $|\mathcal{K}| = k$. Then, upon 
defining
\begin{equation} \label{e:def_block_sparse}
\begin{aligned}
\mathit{\Psi_{\mathcal{K}}} := & \big\{ \bar{\mathbf{X}} = [\bar{\x}^{1},\cdots,\bar{\x}^{P}] \in \mathbb{R}^{N \times P} \quad \text{such that} \\ & \mathbf{\bar{x}}_{i} = \mathbf{0} \hspace{0.1cm} \text{for}  \hspace{0.1cm} i \notin \mathcal{K}, \mathcal{K} \subset [N], \lvert \mathcal{K} \rvert = k  \big\},
\end{aligned}
\end{equation}
the bandlimited signal recovery (and thus also finding the support $\mathcal{K}$) boils down to solving
\begin{equation}
\begin{aligned}
\label{e:opt_support}
& \underset{\mathbf{\bar{X}}}{\text{min}}
& &  \lVert \mathbf{\bar{X}} - \mathbf{\bar{Y}} \rVert_{F}^{2} 
& \text{s.t.}
& &  \mathbf{\bar{X}}\in \mathit{\Psi_{\mathcal{K}}},
\end{aligned}
\end{equation}
where $\bar{\Y} = \V^{\top}\Y $. Note that support recovery is a byproduct of optimizing \eqref{e:opt_support}. 
Inspired by \cite{baraniuk2010model}, we propose to use the $(2,0)$ mixed norm to reformulate \eqref{e:opt_support} 
as
\begin{equation}
\begin{aligned}
\label{e:opt_support_mixed_norm}
& \underset{\bar{\mathbf{X}}}{\text{min}}
& &  \lVert \bar{\mathbf{X}} - \bar{\mathbf{Y}} \rVert_{F}^{2} 
& \text{s.t.}
& &  \lVert \bar{\mathbf{X}} \rVert_{2,0} \leq k,
\end{aligned}
\end{equation}
where the $(p,q)$-mixed norm of matrix $\bar{\mathbf{X}}$ is defined as
\begin{equation} \label{e:mixed_norm}
\lVert \bar{\mathbf{X}} \rVert_{p,q} := \big(\sum_{i=1}^{N} \lVert \bar{\x}^{i} \rVert_{p}^{q} \big)^{1/q}.
\end{equation}
%Note that $(2,0)$ norm counts the number of nonzero rows in $\bar{\mathbf{X}}$.

It follows that the solution $\bar{\mathbf{X}}^{\star}$ of \eqref{e:opt_support_mixed_norm} is obtained 
by the row-wise $l_{2}$-norm thresholding of $\bar{\mathbf{Y}}$. Specifically, upon calculating the 
$l_{2}$-norm of the rows of $\bar{\mathbf{Y}}$ (i.e., $\lVert \bar{\mathbf{y}}_{i} \rVert_2$), we identify the 
$k^{th}$ largest $l_{2}$-norm, $\zeta$. Then, the solution $\bar{\mathbf{X}}^{\star}$ has rows given by

\begin{align} \label{e:support_recovery_solution_form}
\bar{\mathbf{x}}_{i}^{\star}=
\begin{cases}
\bar{\mathbf{y}}_{i} \quad \lVert \bar{\mathbf{y}}_{i} \rVert_2 \geq \zeta, \\
\mathbf{0} \quad \text{otherwise.}
\end{cases}
\end{align}
The running time of finding the solution to \eqref{e:opt_support_mixed_norm} according to \eqref{e:support_recovery_solution_form} is $\mathcal{O}(NP+N \text{log} N)$. This consists 
of finding the $l_{2}$ norm of the rows in $\mathcal{O}(NP)$ and then performing an off-the-shelf 
sorting algorithm (e.g., merge sort) in $\mathcal{O}(N \text{log} N)$.

Analyzing the support identifiability is challenging in the presence of noise. To render it manageable, 
we assume an energy constraint on the noise, i.e., impose a constraint that noise does not exceed 
a threshold $\epsilon_{\mathbf{n}}$. In the following theorem, we provide sufficient conditions for exact recovery of 
the support from the noisy observations assuming an energy-constrained noise model.
\begin{theorem}\label{thm:supn}
Consider the support recovery of $P$ bandlimited graph signals $\mathbf{X} = \mathbf{V} 
\mathbf{\bar{X}} = \mathbf{V} [\bar{\x}^{1}, \cdots, \bar{\x}^{P}] \in \mathbb{R}^{N \times P}$ with 
unknown shared support $\mathcal{K}$ where $\lvert \mathcal{K} \rvert = k$, i.e., $\mathbf{\bar{X}} \in 
\mathit{\Psi_{\mathcal{K}}}$. Let $\mathbf{{Y}} = [\y^{1}, \cdots, \y^{P}] = \mathbf{X} + \mathbf{N}$ 
denote the noisy measurements of the graph signals $\mathbf{X}$, where $\mathbf{{N}} = 
[\n^{1}, \cdots, \n^{P}] \in \mathbb{R}^{N \times P}$ models the noise. Assume $\mathbf{V}$ is 
orthogonal and $\n^{i}$ has bounded $l_{2}$ norm; in particular, $\lVert \n^{i} \rVert_2 \leq \epsilon_{\mathbf{n}}$ 
for all $i \in [P]$. Then
% GFTs $\mathbf{\bar{X}}$ and, as a byproduct, 
 the support $\mathcal{K}$
%are identifiable 
can be exactly recovered
by solving \eqref{e:opt_support} if
\begin{equation} \label{e:support_recovery_condition}
\underset{i \in \mathcal{K}}{\text{min}} \quad \lVert\bar{\x}_i \rVert_2 > 2 \epsilon_{\mathbf{n}} \sqrt{P}.
\end{equation}
\end{theorem}
\begin{proof}
	See Appendix \ref{pf:supn}.
\end{proof}

Inspection of \eqref{e:support_recovery_condition} shows that in the noiseless scenario 
(i.e., $\epsilon_{\mathbf{n}} = 0$), the support is identifiable even for $P=1$. {\color{black}{In the noisy case with $P=1$, if the smallest entry of that one sampled graph signal is greater than $2\epsilon_{\mathbf{n}}$, the proposed framework can still perfectly identify the unknown support from $k$ 
sampled nodes}}. Moreover, in the presence of noise, it 
is apparent that as $P$ grows, the chance of \eqref{e:support_recovery_condition} being 
satisfied increases and the support is rendered identifiable as the number of observations grows; 
see also the numerical tests in Section~\ref{sec:sim}.
%In the following proposition  we show that for the proposed selection sampling scheme in Section \ref{sec:bl} the only required condition for perfect reconstruction with unknown $\K$ (in noiseless setting) is $\V$ having full rank. Further, in contrast to the aggregation sampling method, only $m = k$ noiseless samples are sufficient for perfect reconstruction.
%\begin{proposition}\label{thm:sup}
%	Let $\x = \V\bar{\x}$ be a bandlimited graph signal with unknown support $\K$ such that $|\K| = k$, and let $\hat{\x}$ denote the sampled signal by Algorithm \ref{alg:1}. If $\V$ is invertible, then the original signal  can be recovered from $\hat{\x}$ with $m = k$ samples in noiseless scenario.
%\end{proposition}
%\begin{proof}
%	Since there is no noise, $\y = \x$. Therefore, since $\V$ is invertible, the task of identifying the support  can be cast as the following optimization problem
%	\begin{equation}\label{eq:sub}
%	\begin{aligned}
%	& \underset{\bar{\x}}{\text{min}}
%	\quad \|\bar{\x} - \V^{-1}\y\|_2^2
%	& \text{s.t.}\quad  \|\bar{\x}\|_0 \leq k.
%	\end{aligned}
%	\end{equation}
%It is easy to argue that the optimal solution to this problem is to have $\bar{\x}$
%take the $k$-largest terms from $\V^{-1}\y$ and set the rest to zero. Thus, since there is no noise, $\bar{\x}$ and the unknown support $\K$ can be exactly recovered. Therefore, we can use the results of Section \ref{sec:bl} to acquire $m = k$ samples and the recovery of $\x$ from these samples is guaranteed with probability one, as argued in Theorem \ref{thm:iss}.
%\end{proof}
%The results of Proposition \ref{thm:sup} reveals that when the measurements are noiseless, one can easily recover the support and use Algorithm \ref{alg:1} to sample the graph signal with guaranteed reconstruction performance. In the presence of noise, the task of recovery of the unknown support becomes more challenging and we need to impose some constraints on noise properties to enable identification of $\K$. Specifically, in Proposition \ref{thm:supn}, we provide sufficient conditions to exactly recover the support from noisy observations.  The proposition states   support identification from noisy observations is as easy as the noiseless scenario, as long as the the smallest nonzero entry of $\bar{\x}$ is lager than noise power.
%Naturally, another insightful identifiability result for stochastic noise models would be most valuable, but left as 
%future work.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%=================================== ALGORITHM 2
%\renewcommand\algorithmicdo{}	% removes "DO" from for loops
%\begin{algorithm}[t]
%	\caption{Joint sampling and support recovery}
%	\label{alg:iter}
%	\begin{algorithmic}[1]
%		\STATE \textbf{Input:} $\V$, historical signals $\mathbf{X}$, $m\geq k$, maximum number of iterations $T$.
%		\STATE \textbf{Output:} Subset $S\subseteq \mathcal{N} $ with $|\S|=m$, Support $\K$.
%		\STATE Initialize $t = 0$, $\S^{0} =  [N]$.
%		\WHILE{$t\leq T$}%\vspace{0.1cm}
%		\STATE $t\leftarrow t+1$
%		\STATE
%		$\mathbf{\hat{\bar{X}}} =  \underset{ \lVert \mathbf{\bar{X}} \rVert_{2,0} \leq k}{\text{argmin}}
%		\lVert \mathbf{\bar{X}} - \V_{\S^{t-1},r}^{-1} \mathbf{X} \rVert_{F}^{2} 
%		$%\vspace{0.1cm}
%		\STATE $\K^{t} = \text{supp}(\mathbf{\hat{\bar{X}}})$, $\U = \V_{\K^{t},c}$%\vspace{0.1cm}
%		\STATE Employ Algorithm \ref{alg:1} or Algorithm \ref{alg:greedy} on $\U$ to construct $\S^{t}$.
%		\ENDWHILE
%		\RETURN $\S^T$.
%	\end{algorithmic}
%\end{algorithm}
%%===================================
%%\vspace{-0.5cm}
%\subsection{Joint sampling and support recovery}  
%In Section \ref{sec:rec_hist} we demonstrated that if \eqref{e:support_recovery_condition} is met in the presence 
%of noise, the support is identifiable from $P$ historical samples of the graph signal. After the recovery of support, 
%one can employ Algorithm \ref{alg:1} (Algorithm \ref{alg:greedy}) to construct a sampling set in the non-Bayesian 
%(Bayesian) scenario. In this section, we consider the noisy scenario where the sufficient condition in Section \ref{sec:rec_hist} 
%is not satisfied. Since in this case exact identification of support is not guaranteed, we propose an alternating 
%scheme to jointly identify the support and construct the sampling set in an iterative fashion. Specifically, in the first iteration we set $\S^{0} = [N]$ and identify an approximate support $\K^{1}$ from the historical samples according to the 
%results of Section \ref{sec:rec_hist}, i.e., solve
%\begin{equation}
%\begin{aligned}
%\mathbf{\hat{\bar{X}}} = & \underset{ \lVert \mathbf{\bar{X}} \rVert_{2,0} \leq k}{\text{argmin}}
%& &  \lVert \mathbf{\bar{X}} - \V_{\S^{0},r}^{-1} \mathbf{X} \rVert_{F}^{2} 
%\end{aligned}
%\end{equation}
% and set $\K^{1} = \text{supp}(\mathbf{\hat{\bar{X}}})$. Then, we perform either Algorithm \ref{alg:1} or Algorithm \ref{alg:greedy} on $\V_{\K^{1},c}$ to construct a sampling set $\S^{1}$ such that $|\S^{1}|=m$ in non-Bayesian or Bayesian setting, respectively. This procedure is continued until convergence or meeting a stopping criteria, such as reaching the predetermined maximum number of iterations. This scheme is formalized as Algorithm \ref{alg:iter}.
